Steering a Fleet: Adaptation for Large-Scale, Workflow-Based Experiments

Experimental science is increasingly driven by instruments that produce vast volumes of data and thus a need to manage, compute, describe, and index this data. High performance and distributed computing provide the means of addressing the computing needs; however, in practice, the variety of actions required and the distributed set of resources involved, requires sophisticated "flows" defining the steps to be performed on data. As each scan or measurement is performed by an instrument, a new instance of the flow is initiated resulting in a "fleet" of concurrently running flows, with the overall goal to process all the data collected during a potentially long-running experiment. During the course of the experiment, each flow may need to adapt its execution due to changes in the environment, such as computational or storage resource availability, or based on the progress of the fleet as a whole such as completion or discovery of an intermediate result leading to a change in subsequent flow's behavior. We introduce a cloud-based decision engine, Braid, which flows consult during execution to query their run-time environment and coordinate with other flows within their fleet. Braid accepts streams of measurements taken from the run-time environment or from within flow runs which can then be statistically aggregated and compared to other streams to determine a strategy to guide flow execution. For example, queue lengths in execution environments can be used to direct a flow to run computations in one environment or another, or experiment progress as measured by individual flows can be aggregated to determine the progress and subsequent direction of the flows within a fleet. We describe Braid, its interface, implementation and performance characteristics. We further show through examples and experience modifying an existing scientific flow how Braid is used to make adaptable flows.

==> 5_evaluation_metrics_updated.tex <==
\begin{figure}
    \setlength{\fboxsep}{0pt}
    \includegraphics[width=0.5\textwidth]{figs/metrics_random_loading_100reps.pdf}
    \caption{Metric performance across various datastream sizes}
    \label{fig:metrics}
\end{figure}

Finally, we want to know the time required to evaluate the various metric operations (as enumerated in \autoref{sec:metric-concept}) for various size datastreams. We initialized Braid with datastreams of sizes ranging from 100 to 10,000,000 entries randomizing the order in which values were added to the various datastreams. We then selected a datastream and a metric operation combination to be computed and repeated until each combination had been computed 100 times. We randomize the ordering of sample entry and metric computations  combination to get worst-case results, avoiding caching or other optimizations in the database that might be caused by repeating the same operation consecutively. \autoref{fig:metrics} shows the result of these tests. The most important result is that, even for datastreams of size 1,000,000, any metric can be computed in no more than about 100 milliseconds. Outliers do show up and we attribute these to network delay as a small change in network latency has a signficant impact on transaction times measured in the 10's of milliseconds.

We attribute the generally good performance to Braid's implementation the metrics: each is computed using a single SQL query using a built-in function or, in the case of \texttt{First} and \texttt{Last} a combination of SQL ``ORDER BY'' and ``LIMIT'' clauses. Operations common to flows such as data transfer and computation typically take a minimum of a few seconds, and often minutes or longer, so these times to compute metrics would not have a significant effect on overall flow execution times.


==> proposal_text.tex <==

5.2 Enforce Data Policies. K. Chard (lead), Foster, Liu, Si.

Tradeoffs, such as those just noted, cannot easily be adjudicated by
individual users and administrators. Instead, we need methods for
mapping flows onto continuum resources in ways that satisfy high-level
policies: e.g., response time (“the output of flow F is required
within 10 seconds),” metadata captured (“metadata extractors R and S
must be run on every image”), and data preservation (“outputs A and B
must be staged to persistent storage before an experiment ends”). We
must implement these methods in ways that recognize and address the
fact that some policy goals may be unrealizable at certain times due
to conflicting resource demands.

To permit explicit negotiation of tradeoffs and to avoid catastrophic
failure in such situations, we will architect a Braid policy engine to
translate high-level statements of priority goals into informed
decisions concerning resource allocation, scheduling, and adaptation
(e.g., delay or reduce 8fidelity of reconstruction, replace large data
with summaries). Important research questions include how to express
and implement, concisely, portably, and reliably, distributed policies
concerning where, when, and how data should be analyzed, reduced,
stored, indexed, retained, discarded, etc.

5.2.1 Represent policies.

Our work with application partners suggests a need for policies that
express constraints such as the following on flow
executions. Deadline: a flow must be started or completed by a
particular deadline. Priority: a flow should be prioritized relative
to other flows from the same user or group. Resource usage: a flow
component should not consume more than a predefined limit in terms of
resource allocation used. Locality: computation should minimize data
transfer, favor use of an accelerator, or execute close to an
instrument. Application-specific: for example, an ML model should be
trained until it reaches a threshold metric; or the number of blobs in
an image should be below a threshold.

There is much literature on policy representations [76–79]. We
believe, informed in part by expe- rience with Automate, that
simplicity is vital due to the difficulties in understanding
consequences when complex policies are combined. Braid flows are
essentially a collection of trigger-action rules (e.g., “when data are
obtained from an instrument move for analysis”). Such rules are
advanta- geous for several reasons: they are easy for non-technical
users to use, they enable event-based computation, and they can be
reasoned about and combined with other rules. Such trigger-action
models have long been applied in specific domains, but recently, due
primarily to the growth of IoT devices, they have been adopted widely
for specifying automated behaviors. The web-based IFTTT [44] system is
a well-known example. However, this prior work, including in Automate,
focuses on trigger-action specification rather than constraints and
policies.

To generalize beyond trigger-action, we will develop a rule-based
mechanism for associating constraints and policies with rule
collections. Rule engines (e.g., Drools [80, 81], iRODS [82, 83], SWRL
[84], RBSLA [85]) have long been used for specifying and enforcing
policies, but with com- plex interfaces. We will adopt a simple
JSON-based representation of policies that is similar, and
complementary, to flow representations. An example policy is shown in
Listing 2. As creating policies from scratch can be challenging, we
will develop a set of common policy templates that can be easily
specified by users. We will periodically review use case requirements
and add templates necessary to specify these policies. In most cases
these templates will be fixed, with a set of prede- termined input
values (e.g., runtime, resource utilization); others, however, will
require extensibility to support arbitrary scenarios. In these cases,
we will allow users to define arbitrary constraints based on
information provided to the policy engine (e.g., instrument features,
model accuracy).

5.2.2 Design and implement extensible policy engine.

Our goal is to augment our flows to support scheduling and execution
policies. In order to support many policy types, we adopt a two-tiered
model: simple policies (e.g., deadlines, locality) that apply only
within the scope of a particular flow will be managed as part of flow
execution, while policies that require global knowledge of other
flows, resources, and application-specific features (e.g., priority,
accuracy) will be managed directly by the Braid policy engine. What is
common in both cases is the need to collect information from flows,
flow components, and external systems (instruments, storage, compute,
etc), in order to be considered during flow execution. It is also
important that policy violations be tracked and exposed by the policy
engine such that users are notified of violations immediately in a way
that enables them to investigate the underlying cause.

We will convert simple flow-specific policies into rules that can be
applied directly to a flow.  For example, rules related to deadlines
can be expressed by adding flow components that modify or cancel the
flow during execution. Some flow-level policies may be specified at
the start or end of the flow, while others will need to be decomposed
and wrapped around individual flow components, for example when
restricting execution time for a component. Policies that require
feedback from 9the external action, will require that the augmented
flow consult with the Braid policy engine to make near-real-time
decisions.

When inter-flow knowledge is required, we will develop a new policy
engine capable of tracking properties across flows (while still
adhering to flow access policies), making decisions, and modifying,
suspending, or terminating flows.  Here, flows managed by the same
user, or shared among a group of users, will be controlled (or
influenced) by the policy engine based on defined polices (e.g.,
preference and priority decisions). We will implement this system
using a similar model to the flows system, enabling registration of
policy rules with the scope in which they apply, enabling, automated
and periodic review of flows and system state, and having the ability
to adapt flows execution via calls to the flows management API (on
behalf of authorized users).  In order to collect information needed
for decisions we will develop a queue-based model for making flow and
other external information available to the policy engine. We will use
our existing queues service (originally developed for reg- istering
events) and built upon Amazon’s Simple Queue Service, to reliably
capture and store resource, flow, and application-specific
information. External applications may then be configured to upload
information streams to these queues which may be processed by the
policy engine and used to make decisions on flow state. Such
information may include monitoring (e.g., resource usage, flow
execution, application execution markers) and application-specific
information (e.g., accuracy, training time).

Complex, multi-site, multi-step flows executing subject to various
policies may make it difficult to diagnose (and even detect)
faults. Rather than automate the entire process, past experiences have
shown us that it is crucial that users be notified of errors and
policy violations so that they can manually introspect and diagnose
underlying causes. Our approach here is to ensure that policy
violations are logged as part of the flow state with references to the
specific policies that were violated. We will make this information
accessible to users immediately and at the conclusion of execution. We
will develop APIs for the Braid policy and flows engines to provide
access to the metadata necessary to understand flow state at the level
of individual components and policies as well as the information that
was used to make a particular decision.

